A SoK for SoCs: Reading the TI Leaves on AI for Cyber Threat Intelligence Generation and Sharing

Cyber Threat Intelligence (CTI) is essential for defending mission-critical infrastructure, yet the process of transforming raw attack evidence into shareable CTI remains fragmented and understudied. We conduct a literature survey of academic papers, organizing the CTI lifecycle into three stages: Threat Data Collection, CTI Generation and Sharing, and CTI Consumption. The first and third stages are well represented in the literature, whereas only a small number of papers address CTI Generation and Sharing. To learn how this stage is practiced, we survey practitioners across multiple organizations who routinely generate and share CTI. They describe a largely manual process with four recurring challenges: preventing the exposure of sensitive information, extracting indicators from noisy attack data, correlating observed behavior with standardized tactics, techniques, and procedures (TTPs), and translating CTI into the formats that sharing platforms require. Using the insights from the practitioner survey, we divide the CTI Generation and Sharing stage into four steps: Intelligence Extraction, Normalization and Enrichment, Codification, and Distribution. We then conduct pilot studies that probe the feasibility of current Large Language Models (LLMs) for each step. The pilot studies show that LLMs can assist an analyst in each of the four steps. However, the models recover only a fraction of the indicators the evidence contains, struggle to ground every claim in the supplied evidence, and do not judge what keeps shared intelligence useful to its recipients. Each step therefore requires expert supervision. Based on these observations, we derive three research directions for automating the production of shareable intelligence.

==> Figures/agentic_workflow.tex <==
% --- START: Agentic Workflow Figure (Straight Arrows) ---
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[node distance=0.8cm and 0.7cm]
  
  % --- NODES ---
  
  % TOOLS (top left)
  \node (tools) [titleBox={okabeOrange}, text width=4.2cm]
    {\textsc{Shared Tools} \nodepart{two} {\raggedright\footnotesize
        \texttt{get\_token\_count()}\\
        \texttt{read\_by\_tokens()}\\
        \texttt{spawn\_worker()}\\
        \vspace{1pt}
        \textit{(worker as callable tool)}
    }};
  
  % WORKER (top right, beside Tools)
  \node (worker) [titleBox={gray!60}, right=of tools, text width=3.8cm]
    {\textsc{Worker} \nodepart{two} {\raggedright\footnotesize
        \begin{itemize}[leftmargin=*,noitemsep,topsep=1pt]
          \item Analyzes fragments
          \item Validates claims
          \item Returns insights
        \end{itemize}
        \vspace{1pt}
        \textit{(runs in parallel)}
    }};
  
  % Orchestrator (below Tools, aligned vertically)
  \node (orch) [titleBox={okabeBlue}, below=1.5cm of tools, text width=3.3cm]
    {\textsc{Orchestrator} \nodepart{two} {\raggedright\footnotesize
        \begin{itemize}[leftmargin=*,noitemsep,topsep=1pt]
          \item Entry point
          \item Plans strategy
          \item Spawns workers
          \item Creates PLAN\_V2
        \end{itemize}
    }};
  
  % Analyst (below Worker, aligned vertically and horizontally with Orchestrator)
  \node (analyst) [titleBox={okabeGreen}, below=1.5cm of worker, text width=3.3cm]
    {\textsc{Analyst} \nodepart{two} {\raggedright\footnotesize
        \begin{itemize}[leftmargin=*,noitemsep,topsep=1pt]
          \item Verifies findings
          \item Spawns workers
          \item Refines CTI
          \item Generates output
        \end{itemize}
    }};
  
  % Outputs (bottom, centered between Orchestrator and Analyst)
  \node (outputs) [titleBox={okabeVermilion}, below=of $(orch)!0.5!(analyst)$, yshift=-0.9cm, text width=7.2cm]
    {\textsc{Final Outputs} \nodepart{two} {\raggedright\footnotesize
        \textbf{Structured CTI:} YAML/JSON (IoCs, TTPs, Evidence) \\ 
        \textbf{Export Formats:} MISP, STIX 2.1, Custom Reports
    }};
  
  % --- ARROWS (all straight) ---
  \begin{scope}[on background layer]
    
    % Tool access from Orchestrator (STRAIGHT vertical then horizontal)
    \draw[usesArrow] (orch.north) -- (orch.north |- tools.south);
    
    % Tool access from Analyst (STRAIGHT vertical then horizontal)
    \draw[usesArrow] (analyst.north) -- (analyst.north |- tools.south);
    
    % spawn_worker() invokes Worker (STRAIGHT horizontal)
    \draw[flowArrow, line width=1.3pt, draw=gray!70] 
          (tools.east) -- 
          node[above, font=\footnotesize\bfseries, text=gray!70] {invokes} 
          (worker.west);
    
    % Main workflow: Orchestrator -> Analyst (STRAIGHT horizontal)
    \draw[flowArrow, line width=1.5pt] (orch.east) -- 
          node[above, font=\small\bfseries] {PLAN\_V2} 
          (analyst.west);
    
    % Final output from Analyst (STRAIGHT vertical)
    \draw[flowArrow, line width=1.5pt] (analyst.south) -- (analyst.south |- outputs.north);
    
  \end{scope}
  
\end{tikzpicture}%
}
\caption{Agentic CTI workflow. The \textbf{Orchestrator} plans analysis and creates 
PLAN\_V2; the \textbf{Analyst} verifies and generates structured outputs. 
Both agents use \textbf{Tools} (token counting, file reading) and invoke \textbf{Workers} 
via \texttt{spawn\_worker()} for parallel fragment analysis.}
\label{fig:agentic-workflow}
\end{figure}
% --- END: Agentic Workflow Figure ---

==> Figures/redaction_tradeoff.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[x=5.8cm,y=3.2cm]
  \draw[->,black!70] (0,0) -- (1.05,0);
  \draw[->,black!70] (0,0) -- (0,1.08);
  \node[font=\scriptsize] at (0.55,-0.16) {PII/OII redaction};
  \node[font=\scriptsize,align=center] at (-0.08,1.11) {Attacker\\preserved};

  \foreach \x/\lab in {0/0,0.5/0.5,1/1.0} {
    \draw[black!45] (\x,0) -- (\x,-0.025) node[below,font=\scriptsize] {\lab};
    \draw[black!12] (\x,0) -- (\x,1);
  }
  \foreach \y/\lab in {0/0,0.5/0.5,1/1.0} {
    \draw[black!45] (0,\y) -- (-0.025,\y) node[left,font=\scriptsize] {\lab};
    \draw[black!12] (0,\y) -- (1,\y);
  }

  \draw[cbBlue,thick] (0.39,1.00) -- (0.76,0.21);
  \draw[cbOrange,thick] (0.63,0.42) -- (0.81,0.11);

  \filldraw[cbBlue] (0.76,0.21) circle (2.4pt) node[above right,font=\scriptsize] {GPT-A};
  \draw[cbBlue,thick,fill=white] (0.39,1.00) circle (2.6pt) node[below left,font=\scriptsize] {GPT-U};
  \filldraw[cbOrange] (0.81,0.11) circle (2.4pt) node[below right,font=\scriptsize] {Claude-A};
  \draw[cbOrange,thick,fill=white] (0.63,0.42) circle (2.6pt) node[above left,font=\scriptsize] {Claude-U};
\end{tikzpicture}
\caption{Experiment~3 privacy--utility tradeoff. The x-axis is the mean of PII and OII redaction rates, and the y-axis is attacker-value preservation. A denotes the aggressive prompt and U denotes the utility prompt.}
\label{fig:redaction_tradeoff}
\end{figure}


==> Sections/05_applying.tex <==
\section{Triaging and Applying CTI}\label{sec:triage_apply}

The primary goal of CTI is to provide stakeholders with actionable insights to protect their infrastructure against threats similar to or related to those observed elsewhere.  
Since CTI directly influences security decisions that may alter a network’s defense posture, it is critical to ensure its trustworthiness before adoption.  
First, the CTI must be validated to confirm its authenticity and reliability, as unverified intelligence could lead to ineffective or even harmful security decisions.  
Second, its relevance to the organization's infrastructure must be assessed, as the vast amount of available intelligence needs to be filtered to ensure only actionable and high-priority threats are considered.  
Finally, the validated and prioritized intelligence is applied in the stakeholder’s context to refine security policies, enhance detection mechanisms, and improve overall defensive strategies.  

In this section, we first describe CTI triaging in \autoref{ssec:triaging_cti}, which includes the process of validation and prioritization of CTI.
Then in \autoref{ssec:triage_application}, we explain how CTI is applied within the context of an organization.
Finally, in \autoref{ssec:challenges_cti_application}, we explore the challenges associated with CTI triaging and application, along with potential future directions.

% The main goal of CTI is to communicate key information to stakeholders that can be used to protect their infrastructure against attacks similar to or related to those witnessed by others.
% First, since CTI is used as a basis for taking actions that might change a network's security posture, great is taken to validate the trustworthiness of CTI.
% Second, analyzing the relevance of the information with respect to a specific target infrastructure, as the staggering amount of available intelligence needs to be filtered to a manageable size.
% Finally, the relevant information is used in the stakeholder's context to analyze and possibly change the security mechanisms and policies currently deployed. 
% In this section, in \autoref{ssec:triage_validate} er first explain how the validation step is carried out, then in \autoref{ssec:triage_prioritization}) we go over how the CTI is prioritized, finally in \autoref{ssec:triage_application} we describe the process of applying  CTI with context of an organization. 

% In this section, we explain the various stages involved in this process. 




% There are three considerations involved when receiving CTI, which will be covered in the following sections.
% First, during the validation phase assesses if the CTI be trusted~(\autoref{ssec:triage_validate}).
% Next, the organization receiving this validated CTI would consider how to prioritizate it~(\autoref{ssec:triage_prioritization}).
% Finally, the prioritized CTI is strategically applied according to the needs of the organization~(\autoref{ssec:triage_application})
% %
% The section concludes by highlighting the opportunities for the application of AI techniques to achieve greater effectiveness (\autoref{ssec:challenges_cti_application}).



% Since CTI is used as a basis for taking actions that might change the security posture of a network, great care should be taken to validate the trustworthiness of CTI.
% A second step involves analyzing the relevance of the information with respect to a specific target infrastructure, as the staggering amount of available intelligence needs to be filtered to a manageable size.
% Finally, the relevant information is used in the stakeholder's context to analyze and possibly change the security mechanisms and policies currently deployed. 
%


%Taking action on CTI provided by others involves three phases: 1) verifying the trustworthiness of the CTI, 2) prioritizing the relevance of the information in the context of the specific environment, and 3) applying the necessary actions to safeguard against the threat.
%The following subsections discuss each of these phases.

\subsection{Triaging CTI}
\label{ssec:triaging_cti}
\sv{Todo:
\\
1. We should definitely talk about threat modelling here. There are papers that try to find vulnerabilities within the organization. but we need to highlight that these work do not correlate the information obtained to prioritize threat.
\\
2. We need to mention that most of the existing widely used threat sharing and management framework expects the receiver to validate the threats. Some of them do provide a community driven scoring system, where others can rate the feed.
\\
3. Currently validating is a pain, existing work provide methodology to validate feeds (how reputation is built), but they do not really explore how to actually validate the threats. Decreasing the applicability of these works. They expect that there already exists a methodology to validate. 
\\
4. Applying CTI: Detail threat intelligence platform properly. 
}
% Cyber Threat Intelligence (CTI) plays a critical role in defending organizations against cyber threats, but its effectiveness depends on proper triaging.  
Given the vast amount of intelligence generated from various sources, security teams must determine whether a piece of intelligence is trustworthy, applicable, and worth acting upon~\cite{sillaber2016data,zibak2022threat,  geras2024big}. 
One straightforward approach to selecting a CTI source is volume-based selection, where the source is chosen based on the quantity of intelligence it provides. 
The goal is to maximize coverage~\cite{jung_empirical_2004,kuhrer2014paint, sheng_empirical_2009, levchenko_click_2011, pitsillidis_tasters_2012}. 
This method is particularly useful for shared email addresses, domain names, and IP address blacklists, where maintaining a large set of indicators improves detection and false positives have a relatively low impact.

However, when CTI describes an attack's tactics, techniques, and procedures, false positives can significantly disrupt operations, making volume-based selection less effective. 
In such cases, organizations perform triaging to ensure that intelligence is accurate, contextually relevant, and actionable~\cite{geras2024big}. 
The triaging process consists of three key steps: validation, which ensures intelligence is credible; relevance assessment, which determines whether the intelligence applies to the organization’s infrastructure; and impact-based prioritization, which helps allocate security resources effectively based on the severity of the threat.

\mypar{Validating CTI.}  
The goal of this step is to ensure that the intelligence is credible and actionable before integrating it into security operations.
Although there have been attempts to formally define the quality of CTI sources ~\cite{sakellariou_methodology_2024, liao2016acing}.
Organizations primarily use two methods for validation: reputation-based validation and redundancy-based validation~\cite{geras2024big}.  

Reputation-based validation establishes trust in CTI sources based on their historical accuracy and reliability.  
Organizations rely on a combination of historical detection accuracy, real-time feedback loops, and correlation with real-world incidents to determine a source’s reputation.
Platforms such as \textit{VirusTotal}~\cite{VirusTotal} and \textit{MISP}~\cite{Wagner2016MISPTD} integrate analyst reviews, allowing security professionals to rate intelligence based on its reliability.  
Furthermore, reputation is assessed at both the source level and IoC level.  
At the IoC level, reputation evolves dynamically—new indicators receive neutral scores, which increase if the indicator is observed in real-world attacks and decrease if found to be benign~\cite{sakellariou_methodology_2024, liao2016acing, wang2022comprehensive, qiang2018quality }. 
A recent study has shown that high-reputation CTI feeds contain significantly less overlap in intelligence~\cite{bouwman2020different}.  Therefore, rather than providing redundant data, trusted sources contribute unique, high-value intelligence, making reputation-based validation essential for broadening CTI coverage while ensuring accuracy.  
% This also challenges the assumption that redundancy alone is an effective validation strategy, as **some of the most critical threat intelligence is not widely reported** across multiple feeds.  


Redundancy-based validation is a fundamental approach to ensuring the credibility of cyber threat intelligence by cross-referencing intelligence, often in the form of IoCs, across multiple independent sources. When the same IoC appears consistently in different feeds, confidence in its reliability increases~\cite{kuhrer2014paint, meier2018feedrank, gao2018graph, sakellariou_methodology_2024}. This approach helps filter out noise, identify widely recognized threats, and strengthen the reliability of shared intelligence.

Security teams rely on redundancy to verify IoCs before integrating them into detection and response workflows. 
Weighted redundancy models assign greater importance to high-credibility sources (e.g., national CERTs, top-tier security firms), while lower-confidence sources require further validation. 
Additionally, cross-source validation plays a crucial role in determining intelligence trustworthiness by analyzing how different vendors report a given threat. 
For instance, a domain reported as malicious by \textit{CrowdStrike}, \textit{Mandiant}, and \textit{Recorded Future} carries significantly more weight than an IoC flagged solely in an unverified open-source blog post.
However, redundancy is not always a strong indicator of value. 
Some threats, such as advanced persistent threats (APTs), are highly targeted and may only be reported by select intelligence vendors rather than appearing in multiple feeds. 
% Conversely, commodity threats that appear in several sources may be outdated or irrelevant, leading to unnecessary blocking.
While redundancy strengthens confidence in intelligence, security teams must refine their validation techniques to mitigate these challenges.
% Redundancy-based validation ensures intelligence credibility by cross-referencing intelligence (often in the form of IoCs) across multiple independent sources.  
% If the same IoC appears consistently in different feeds, confidence in its reliability increases~\cite{kuhrer2014paint, meier2018feedrank,gao2018graph, sakellariou_methodology_2024}.  
% However, redundancy is not always a strong indicator of value.  
% Some threats, such as advanced persistent threats (APTs), are highly targeted and may only be reported by select intelligence vendors rather than occurring in multiple feeds.  
% Additionally, commodity threats that appear in multiple sources may be outdated or irrelevant, leading to unnecessary blocking.  
% Security teams address these limitations by applying weighted redundancy models, where high-credibility sources (e.g., national CERTs, top-tier security firms) receive greater weighting, while low-confidence sources require further validation.  
% Organizations also perform cross-source validation, analyzing how intelligence is reported across different vendors.  
% For example, a domain reported as malicious by \textit{CrowdStrike}, \textit{Mandiant}, and \textit{Recorded Future} carries more weight than an IOC flagged only in an unverified open-source blog post.  

\mypar{Relevance Assessment.}  
Once validated, CTI must be assessed for its relevance to an organization’s security posture~\cite{wagner2017relevance, de2023no, cabana2021threat}.  
A validated threat may be inapplicable if it does not align with the organization’s infrastructure or threat model.
For instance, if intelligence reports a Windows-based ransomware strain, but an organization only operates Linux systems, the intelligence has low relevance.  
To systematically determine the relevance of CTI, security teams assess whether their infrastructure is exposed to the vulnerabilities being exploited. 
If a newly detected exploit, such as a Log4j vulnerability, is reported, but the organization does not use Log4j-based software, the intelligence is deprioritized since it does not pose an immediate risk. 

% \mypar{Impact-Based Prioritization.}
\mypar{Impact-Based Prioritization.}
After validation and relevance assessment, organizations prioritize threats based on exploitability, potential damage, and real-world activity~\cite{sillaber2016data, li2019reading}. 
A zero-day vulnerability with public exploit code is more critical than a complex, multi-stage attack. 
Similarly, a supply-chain compromise affecting critical infrastructure presents a greater risk than adware on non-sensitive endpoints. 
To enhance prioritization, organizations leverage CVSS scoring~\cite{cvssv4} to assess a vulnerability’s severity and Known Vulnerability Validation (KVV)~\cite{cisaKEV} to determine its actual impact within their environment. Threats actively exploited in real-world incidents, such as ransomware strains observed in multiple attacks, are prioritized over theoretical exploits. By continuously evaluating these factors, security teams focus resources on the most pressing threats.
% Additionally, relevance is evaluated based on the organization's ability to detect and respond to the reported threat. 
% For instance, if intelligence indicates that an attack relies on malicious PowerShell execution, but the organization lacks logging mechanisms to monitor PowerShell activity, it may be blind to the attack. 
% This highlights gaps in security visibility and may necessitate adjustments in monitoring strategies to ensure effective threat detection.

% - Historical Attack Correlation: Has the organization been targeted by similar adversary techniques before?  
%   - If an organization was previously attacked by a ransomware group, any new intelligence linked to that group becomes immediately relevant.  

% Security teams also analyze adversary targeting patterns.  
% Some threat groups specialize in targeting specific industries (e.g., FIN7 targeting financial institutions), making intelligence more relevant for organizations in that sector.  
% However, if evidence suggests an attack is expanding to new industries, security teams reassess its relevance.



% When an organization receives Cyber Threat Intelligence (CTI), validating its accuracy and relevance is crucial before integrating it into security measures~\cite{geras2024big, zibak2022threat, sillaber2016data}.  
% Failure to validate CTI can lead to false positives, overlooked threats, and inefficient resource allocation.  
% This validation process ensures that intelligence is actionable and aligns with real-world threats.  

% Industry validation primarily relies on continuous monitoring, cross-referencing with historical incidents, and feedback loops from operational security systems.  
% Organizations assess intelligence reliability by tracking false positives, evaluating detection efficacy, and refining reputation scores dynamically using machine learning models and heuristics.  
% Threat scoring is a widely used technique, assigning a reputation score to entities such as IPs, domains, or file hashes based on their historical behavior and recurrence in attack campaigns.  
% These reputation scores are cross-validated against threat telemetry collected from firewalls, SIEMs, IDS/IPS, and endpoint security solutions.  
% Sandboxing techniques further test and classify suspicious entities before integrating them into security controls.  

% To enhance accuracy, organizations leverage crowdsourced intelligence sharing and feedback mechanisms.  
% Platforms such as VirusTotal, MISP, and commercial CTI exchanges (e.g., Recorded Future, CrowdStrike Falcon X) integrate community feedback to refine reputation scores.  
% An initially low-confidence threat indicator gains credibility as multiple organizations confirm its malicious nature, while misclassifications are corrected through analyst reviews or automated feedback loops.  
% Additionally, reputation decay mechanisms prevent outdated intelligence from remaining indefinitely classified as high-risk, ensuring that intelligence remains relevant.  
% Historical attack pattern analysis, particularly mapping threats to MITRE ATT\&CK techniques, further enhances validation by correlating indicators with past adversary behaviors.  

% In academia, research has proposed structured methodologies for validating CTI.  
% Formal quality assessment frameworks~\cite{sakellariou_methodology_2024, liao2016acing} evaluate intelligence based on redundancy, data volume, and source reputation.  
% Several studies prioritize data redundancy, assuming that intelligence corroborated by multiple independent sources is more reliable~\cite{kuhrer2014paint}.  
% However, in high-security domains such as finance and government, uniqueness is often prioritized over redundancy, as more evasive threats are typically detected by well-resourced organizations with specialized expertise~\cite{bouwman2020different}.  
% Machine learning and NLP techniques have been employed to extract high-quality intelligence from expert discussions and open-source platforms~\cite{paladini2024you, huang2017gossip}, demonstrating promising results in filtering out irrelevant or erroneous data.  


%%%%
% \subsection{Validating CTI}\label{ssec:triage_validate}
% When an organization receives Cyber Threat Intelligence (CTI), it's crucial to first assess the credibility and relevance of the information before integrating it into their security measures~\cite{geras2024big, zibak2022threat, sillaber2016data}. 
% Not all CTI is sourced from trusted organizations, as described in the motivating example in~\autoref{ssec:framework_motivating_example}. 
% Consequently, imprecision in the CTI generation process may introduce irrelevant or erroneous data, leading to false positives and reduced effectiveness.
% Therefore, validation is a critical step to ensure that decisions are based on accurate and relevant intelligence, preventing unnecessary disruptions and misallocation of resources.

% Although there have been attempts to formally define the quality of CTI sources (~\cite{sakellariou_methodology_2024, liao2016acing}), organizations validate incoming CTI by assessing the \textit{quality} of the data being provided the \textit{ redundancy} of the information between multiple sources or the \textit{ reputation} of the source.
% % Although there have been attempts to formally define the quality of CTI sources (~\cite{sakellariou_methodology_2024, liao2016acing}), organizations validate incoming CTI by assessing the \textit{volume} of the data being provided, the \textit{ redundancy} of the information between multiple sources or the \textit{ reputation} of the source.

% Several well-documented approaches have prioritized the volume of data in a feed as a heuristic for broader coverage~\cite{jung_empirical_2004,kuhrer2014paint, levchenko_click_2011, pitsillidis_tasters_2012, sheng_empirical_2009}.
% This perspective originates from the era of shared email blacklists, where having a larger list was often seen as beneficial, as missing a spam domain could be more problematic than the occasional false positive. 
% However, while volume can contribute to coverage, modern threat intelligence places greater emphasis on data quality, accuracy, and contextual validation to ensure actionable insights.

% % Several well-documented approaches prioritize the \textbf{volume} of data in a feed~\cite{jung_empirical_2004,kuhrer2014paint, levchenko_click_2011, pitsillidis_tasters_2012, sheng_empirical_2009}.
% % The rationale behind this approach is rooted in the days of shared email blacklists, where a larger list was inherently better and a false positive was merely an inconvenience.
% Validation of an IoC found in multiple sources (\textbf{redundancy}) works well when considering large lists and there is a low cost for false positives~\cite{kuhrer2014paint}. 
% However, a more sophisticated redundancy-based validation is required when a false positive is not acceptable.
% In such cases, NLP and ML processing of expert online discussion forums can yield high-quality data~\cite{paladini2024you,huang2017gossip}.

% In some sectors, such as finance and government, 
% % there is another marketplace where 
% the demand for high-quality data eclipses the desire for a long list of potential IOCs.
% Although, intuitively, multiple independent reports on a piece of intelligence should contribute to the reliability and accuracy of the data~\cite{li2019reading}, the perception in the threat intelligence community is that often the data (CTI) that is ubiquitous has less value and is easier to obtain.
% The assumption is that the intelligence associated with more sophisticated and evasive threats will be extracted only by [reputable?] organizations with access to substantial human expertise and computational resources.
% As a result, the uniqueness of the CTI data is a value. 

% In this marketplace, the \textbf{reputation} of CTI providers is associated with a higher market price for Paid Threat Intelligence (PTI) data.
% A recent survey of security professionals who use PTI found that organizations tolerate limited coverage and a small number of reports as long as the TI remains free of false positives.
% Among top PTI sources, data overlaps minimally, with little duplication between commercial and public sources~\cite{bouwman2020different}.
% However, this model presents a risk: the most critical threats, which are often difficult to detect or validate, may be excluded.

% This observation challenges the notion that more information is better and highlights the value of high-quality data over large quantities of data.
% Nevertheless, focusing on quality and reducing false positives comes with trade-offs.
% Market research indicates that customers often struggle to compare different PTI sources effectively~\cite{kuhrer2014paint}.
% A recent study found that PTI coverage is limited, with less than 10\% overlap between top sources --showing that the effort to compare sources is of limited value~\cite{bouwman2020different}.

% We see that redundancy rarely occurs when reputation is at stake, and the market demand for high-quality feeds has led to smaller, more specialized datasets.
% The contrasting motivations of redundancy and reputation suggest a need for a new mechanism to share and validate CTI.
% Ideally, such a platform would incorporate the trustworthiness of sources while also emphasizing the redundancy of threats identified by multiple sources.


%% ORignal prioritization
% \subsection{Prioritization}\label{ssec:triage_prioritization}
% % \ns{Integrate - \cite{cabana2021threat} sophisticated packet analysis. - \cite{de2023no} selective attention. \cite{li2019reading} - metrics to evaluate threat intelligence data feeds \cite{sillaber2016data} - timely updates and removal of outdated information}
% Once the trustworthiness of Cyber Threat Intelligence (CTI) is validated, organizations must prioritize this intelligence to ensure it is actionable and relevant to their specific security environment.
% % Along with assessing the trustworthiness of the CTI, the organizations must also evaluate whether the CTI is relevant for their organizations infrastructure, and asses the impact of the threat. 

% Prioritization is essential to manage limited resources effectively and to mitigate the risk of unintended consequences from applying CTI.
% Two primary approaches to prioritizing CTI are \textit{effect}-based and \textit{relevance}-based assessments.

% In \textbf{effect}-based prioritization, CTI is ranked according to the potential consequences of acting on the intelligence information.
% Organizations make an assessment of the actions that would be triggered by the CTI and evaluate the possible damage that could occur if intelligence were manipulated or poisoned.
% A ranking system is used to limit the impact of erroneous CTI~\cite{li2019reading, sillaber2016data}.
% For example, if applying a specific piece of CTI would result in blocking critical services or isolating important infrastructure, that intelligence receives closer scrutiny and is treated with caution.
% This approach helps minimize disruptions to the organization's operations and aims to ensure that security measures do not inadvertently create vulnerabilities or disrupt business.

% To implement effect-based prioritization, organizations can use decision models that weigh the benefits of applying CTI against potential risks.
% By considering the downstream effects of taking action, security teams can make informed choices about which intelligence to act on and which to continue monitoring.

% \textbf{Relevance}-based prioritization assesses how applicable CTI is to the organization's specific environment~\cite{wagner2017relevance, de2023no, cabana2021threat}.
% CTI that describes threats or attacks targeting services or platforms not present in the organization's network is deprioritized or even discarded~\cite{de2023no}.
% For example, intelligence about a widespread attack on a database technology not deployed within the organization holds little value and does not warrant immediate attention.
% On the other hand, CTI related to attacks that exploit software or configurations prevalent at the edge of the organization's infrastructure receives higher priority~\cite{cabana2021threat}.

% This method ensures that security resources are focused on protecting against threats that pose the most significant risk to the organization.
% Relevance-based prioritization also enables teams to filter out noise from CTI feeds, reducing the volume of intelligence that requires analysis and action.
% By tailoring CTI to the organization's environment, security teams can create a more efficient and effective threat response strategy.

% In practice, these two prioritization methods have competing concerns---if CTI is not relevant (and narrowly targeted) it has no effect; if it is relevant, it has some effect.
% Effect-based assessments safeguard against potential damage from poisoned or manipulated CTI, while relevance-based assessments ensure that resources are focused on applicable threats.
% These competing concerns need to be balanced, and we propose that AI could be well-suited to balance these concerns.

% \subsubsection{Opportunities for AI}

% AI can assess the effect of validated CTI by simulating the outcomes of various response strategies and their outcomes.
% . risk and potential impact of acting on specific CTI 
%% ORignal prioritization

\subsection{Applying CTI}  
\label{ssec:triage_application}
Once CTI is validated for accuracy and assessed for its potential impact, the focus shifts from validation to practical application: understanding how this intelligence fits within the organization's security posture and how it can be leveraged to enhance defense mechanisms.  
Applying CTI is particularly challenging due to the vast volume of intelligence data and the dynamic nature of both the threat landscape and an organization’s network infrastructure.  

To address these challenges, security teams rely on Threat Intelligence Platforms (TIPs) and internal knowledge bases (KBs) to centralize and correlate CTI data.  
These platforms provide structured storage for multiple CTI sources~\cite{shu2018threat}, including IoC feeds, blog posts, reports, and alerts, which are processed through feed-specific plugins that extract relevant information.
While encoding structured threat intelligence is straightforward for machine-readable formats, processing natural language reports or unstructured log data remains a challenge.  
Academic research has explored various approaches to automate this process, extracting CTI information from online and darknet forums~\cite{paladini2024you, zhu2018chainsmith, huang2017gossip}, OSCTI feeds~\cite{gao2021enabling, gao2021system}, and threat reports~\cite{dekel2022mabat, alam2023looking, Rani2024TTPXHunterAT, kaiser2023attack, fieblinger2024actionable, zhao2020cyber, husari2017ttpdrill, rani2023ttphunter}.  
By leveraging TIPs and KBs, organizations can systematically apply CTI through four key aspects.  

First, validated CTI must be correlated with existing intelligence to assess its relevance and historical context. 
This involves using TIPs and knowledge graphs to determine whether the identified IoCs, or TTPs have been previously observed in other incidents.  
For example, if an IP address involved in a new phishing campaign was previously associated with an infrastructure for the distribution of credential-stealing malware, TIPs link these two components and allow security analysts to attribute them to the same threat actor~\cite{husari2017ttpdrill, rani2023ttphunter}. 
%Once ingested, TIPs enable correlation by linking multiple reports that mention the same IOCs like malware file hash or refer to the same domain name~\cite{husari2017ttpdrill, rani2023ttphunter}.  
By tracking the evolution of adversary behaviors, analysts can establish patterns and anticipate potential attacks.  

Second, organizations must evaluate whether the CTI is applicable given their existing security infrastructure.  
For instance, if a new threat involves malicious PowerShell execution, defenders must assess whether they have visibility into PowerShell activity.  
If the necessary monitoring capabilities are absent, implementation may require new logging mechanisms, additional storage capacity, or third-party security solutions.
This feasibility assessment is currently carried out manually, making it a time-consuming process that depends on the organization's existing capabilities.  
Despite its critical role in operationalizing CTI, there has been little to no academic research focused on automating this assessment, leaving a gap in systematic approaches to evaluating security readiness.

Third, assuming the necessary telemetry and log collection mechanisms are in place, security teams must determine whether their detection systems would successfully identify the threat.
This activity, called efficacy analysis, answers the question: \textit{Would I detect this attack if it would happen in my network?} 
While TIPs can provide some support in determining the coverage of existing detection mechanisms (e.g., IDS signatures associated with CVEs), currently this is a mostly manual effort that requires an understanding of the capabilities of the various detection components of a network and the overall ability of an organization to correlate multiple security events.
Academic research has explored methods for correlating disparate events and IoCs, as well as mapping them to known attack patterns and TTPs~\cite{zhao2020cyber, zhu2018chainsmith, gao2021enabling, alam2023looking}. 
However, operationalizing these insights within real-world detection workflows remains largely a manual and expertise-driven process, limiting automation in efficacy analysis.

%This step is closely linked to \textit{threat hunting}—if current detection rules are insufficient, analysts must manually investigate log sources, refine detection logic, or develop new signatures to cover the identified tactics and techniques.  

Fourth, TIPs help security analysts in answering an essential question: \textit{Is this attack happening (or has already happened) in my network?} 
This is especially important when the previous task has identified blind corners in an organization's detection capabilities. 
This task, often called \textit{threat hunting} is supported by TIPs by correlating CTI with historical and real-time log data, looking for signs of ongoing or past intrusions~\cite{liao2016acing, husari2017ttpdrill, rani2023ttphunter}.  
If related IoCs have already appeared in network traffic, endpoint logs, or authentication records, immediate incident response actions may be required.  

Applying CTI is an iterative process that continuously refines security postures by improving detection capabilities and response strategies.  
By systematically addressing these four aspects, organizations can ensure that CTI is actionable, relevant, and effectively integrated into their defense operations.  

% A second common use of TIPs is through integration with software inventory and vulnerability scanning tools.
% These tools provide a view of the components and services deployed in an infrastructure, which allows a TIP to identify CTI data that is highly relevant to a specific infrastructure, allowing for effective CTI triaging.
% The simplest approach matches the vulnerable products mentioned in a CVE record mentioned in a report with the software deployed in the organization's network, but AI could enable more sophisticated processing where the multi-step attack patterns mentioned in a threat report are directly mapped to an infrastructure's components to understand the feasibility of a similar attack in the local context.

% Another common application of TIPs is through integration with malware analysis environment and signature evaluation system. 
% In this case the goal is to answer the question: ``If this attack would happen in my infrastructure, would I be able to detect it?''
% Automating this task is challenging, as it requires the automatic downloading of malicious artifacts, the reproduction of network-based attacks, and the analysis of the combined results. 
% Approaches based on LLM agents have shown promise in the creation of exploits, but more work needs to be done to effectively leverage CTI data to automatically determine the detection efficacy and threat coverage of an organization's security infrastructure.

% The fourth application of TIPs is the use of CTI for threat hunting in the local context.
% By integrating with the logs collected by network and host monitoring tools (often stored in large log management systems) with CTI, it is possible to support the identification of attacks in an organization's network based on information contained in CTI reports.
% This is the main goal of CTI itself: using pre-existing information about cyber threats to detect and mitigate the attacks in an organization's network.
% At the moment this is largely a manual process, and TIPs work as support for SOC analysts and threat hunters.
% However, there is a great opportunity to use AI-based techniques in order to enhanced manual analysis (e.g., by providing a RAG-based contextualization of network events based on CTI) or to automatically understand if the evidence of instances of attacks described in CTI feeds is actually present in an organization's network. 
%%%
% By leveraging knowledge graphs and historical threat intelligence, analysts can track the evolution of adversary behaviors and establish connections between seemingly unrelated attacks.  
% For example, if an IOC from a new phishing campaign was previously linked to a credential-stealing malware, this information helps defenders anticipate potential attack vectors.  



% Second, organizations must evaluate whether the CTI is applicable given their current security infrastructure.  
% For instance, if a new threat involves malicious PowerShell execution, defenders must determine whether they have the capability to monitor PowerShell activity.  
% If not, implementing such monitoring may require new logging mechanisms, additional storage capacity, or third-party security solutions.  
% The feasibility of applying CTI depends not only on its relevance but also on the organization's ability to act upon it.  

% Third, assuming the necessary resources for log collection are in place, security teams must assess whether their existing detection mechanisms would successfully identify the threat.  
% This step is closely linked to \textit{threat hunting}. 
% That is if the current detection rules would fail to flag the attack, analysts must manually investigate log sources, refine detection strategies, or develop new signatures to cover the identified tactics and techniques.  

% Finally, an essential question remains: \textit{Is this attack already happening?}  
% By correlating validated CTI with historical and real-time log data, organizations can identify signs of an ongoing or past intrusion.  
% If related IOCs have already been observed in network traffic, endpoint logs, or authentication records, immediate incident response actions may be required.  

% Applying CTI is not a passive process but an iterative approach that strengthens security postures by continuously refining detection capabilities and response strategies. By systematically addressing these four aspects, organizations can ensure that intelligence is actionable, relevant, and effectively integrated into their defense operations.  
% Applying Cyber Threat Intelligence (CTI) effectively means transforming validated insights from various threat intelligence feeds into actionable strategies that strengthen an organization's overall cyber defense posture. CTI enables organizations to identify, prioritize, and respond to threats in a dynamic landscape by leveraging Indicators of Compromise (IOCs) as critical building blocks.
% Although IOCs can be extracted from traditional blacklists, such as CleanMX \cite{cleanmx} and PhishTank \cite{phish_tank}, these sources typically follow openIOC standards and cover only a limited range of IOC classes, without revealing relationships or providing contextual information~\cite{liao2016acing}. 
% In contrast, IOCs from technical blogs and forums are more valuable to security practitioners due to their detailed attack descriptions. 
% However, extracting CTI from these unstructured sources has traditionally been manual and labor-intensive, posing scalability challenges for human analysts. 

% CTI sources consist of machine-consumable formats like STIX, as well as unstructured (e.g., emails, blogs) and structured texts (e.g., threat reports). To utilize these feeds, indicators such as IP addresses, domain names, and MD5 hashes are extracted and organized into a knowledge base. 
% This process involves identifying relationships between IOCs, modeling adversary behavior, and mapping findings to frameworks like MITRE ATT\&CK \cite{mitre_attack} and the Pyramid of Pain \cite{bianco2013pyramid}. 
% Recent advancements in Natural Language Processing (NLP) have automated the extraction of attack information from forums \cite{paladini2024you, zhu2018chainsmith, huang2017gossip}, OSCTI feeds \cite{gao2021enabling}, and threat reports \cite{dekel2022mabat, alam2023looking, Rani2024TTPXHunterAT, kaiser2023attack, fieblinger2024actionable, zhao2020cyber, husari2017ttpdrill, rani2023ttphunter}. 
% These advancements convert data into machine-readable formats, enabling actionable CTI applications, as detailed below.

% \mypar{Threat Detection.}
% Threat detection focuses on identifying and mitigating potential breaches before they escalate, minimizing risks, and bolstering organizational defenses. 
% CTI is used to create detection rules and blacklists based on IOCs and their relationships, such as TTPs and IOC dependencies. 
% These rules are implemented in Intrusion Detection Systems (IDS) and Security Information and Event Management (SIEM) systems, which monitor network activity in real time. 
% Alerts generated by these systems are reviewed by analysts to refine detection mechanisms further. 
% Additionally, AI-driven detection systems use anomaly detection and behavioral analysis to complement traditional methods, improving accuracy and reducing false positives.

% \mypar{Threat Hunting.}
% Threat hunting leverages CTI to proactively uncover unknown threats, contrasting with the reactive nature of threat detection. 
% This exploratory, hypothesis-driven process involves analyzing IOCs, TTPs, and patterns to identify malicious activities. 
% Proactive threat hunting hypothesizes attack scenarios without waiting for alerts, while reactive hunting investigates alerts to uncover deeper threats. 
% Tools such as eXtended Detection and Response (XDR) solutions and Security Orchestration, Automation, and Response (SOAR) systems play a critical role in data collection and analysis. 
% Frameworks like MITRE ATT\&CK guide analysts in mapping adversary behavior and prioritizing findings.

% \mypar{Incident Response.}
% Incident response focuses on managing confirmed security incidents to minimize impact and prevent recurrence. 
% CTI provides essential insights into threat actor behaviors, TTPs, and behavior graphs, enabling organizations to identify the nature and scope of incidents. 
% These insights guide containment, eradication, and recovery strategies, ensuring effective resolutions while preserving evidence for forensic analysis. 
% Unlike detection and hunting, incident response emphasizes post-incident learning to improve future defenses.

% \mypar{Risk Management.}
% Risk management uses CTI to identify and address emerging threats by analyzing unstructured data, trends of threat actors, and evolving attack techniques. 
% CTI supports the development of proactive strategies, including threat modeling, vulnerability prioritization, and mitigation planning. 
% These strategies involve simulating attack scenarios, improving situational awareness, and automating defenses to effectively address new risks.

% \mypar{Security Awareness and Training.}
% Security awareness programs use CTI to educate employees about real-world threats with insights into TTPs observed in recent attacks. 
% These programs include phishing simulations, scenario-based exercises, and role-specific training aligned with frameworks like the NIST Cybersecurity Framework. 
% Despite advancements in CTI tools, there remains a gap in automated systems to generate dynamic training content based on evolving threat patterns -- highlighting an area for future research.

% \subsection{Applications of CTI}
% Applying Cyber Threat Intelligence (CTI) effectively means transforming validated insights from various threat intelligence feeds into actionable strategies that strengthen an organization's overall cyber defense posture. 
% At the core of CTI are IOCs, which serve as critical building blocks in identifying and mitigating threats. 
% Although IOCs can be extracted from traditional blacklists, such as CleanMX \cite{cleanmx} and PhishTank \cite{phish_tank}, these sources typically follow openIOC standards and cover only a limited range of IOC classes and do not reveal the relationships between IOCs or provide contextual information~\cite{liao2016acing}. 
% In contrast, IOCs extracted from articles in technical blogs and forums are more valuable to security practitioners, as they often include comprehensive attack descriptions. However, the process of extracting CTI from these unstructured sources has traditionally been manual and labor-intensive. 
% The high volume of information from these sources poses scalability challenges, making it difficult for human analysts to process them efficiently and cost-effectively.
% CTI sources include not only machine-consumable formats like STIX but also unstructured text (e.g., emails, blogs) and structured text (e.g., threat reports) from various sources. 
% To utilize text-based CTI feeds, indicators such as IP addresses, domain names, and MD5 hashes must first be extracted and organized into a knowledge base. This involves identifying relationships between IOCs, modeling adversary behavior, and mapping them to established frameworks like MITRE ATT\&CK \cite{mitre_attack} and the Pyramid of Pain \cite{bianco2013pyramid}. 

% Recent advancements in Natural Language Processing (NLP) have enabled the automated extraction of attack information from online forums \cite{zhu2018chainsmith}, open-source cyber threat intelligence (OSCTI) feeds \cite{gao2021enabling}, and threat reports \cite{dekel2022mabat, alam2023looking, Rani2024TTPXHunterAT, kaiser2023attack, fieblinger2024actionable, zhao2020cyber}. 
% These techniques convert data into machine-readable formats, build knowledge bases, identify attack patterns \cite{gao2021enabling, alam2023looking}, and prioritize artifacts for analysis \cite{dekel2022mabat}. 
% Once organized, this actionable CTI can be applied in various domains, including threat detection, threat hunting, incident response, countering emerging threats, and security awareness.
% Below we explain each application of CTI in detail.

% \mypar{Threat Detection.}
% Threat detection focuses on identifying and mitigating potential breaches before they escalate, thereby minimizing risks and strengthening organizational defenses. In this context, CTI is used to create detection rules and blacklists based on IOCs and their relationships, such as TTPs and IOC dependencies. 
% These detection rules are implemented in Intrusion Detection Systems (IDS) and Security Information and Event Management (SIEM) systems, which monitor and analyze network activity in real-time. When a match is found, alerts are generated and reviewed by analysts. 
% Additionally, firewalls and endpoint protection systems leverage CTI to block known malicious activities preemptively. 
% Emerging AI-driven detection systems complement traditional rules-based approaches by using anomaly detection and behavioral analysis to identify previously unknown threats.
% This combination enhances the effectiveness of detection mechanisms and reduces false positives.

% \mypar{Threat Hunting.}
% Unlike threat detection, which primarily focuses on real-time decision-making based on predefined rules, threat hunting leverages CTI to proactively uncover unknown threats. 
% It is an exploratory and hypothesis-driven process where analysts investigate potential adversary activities within the organization’s network.
% Threat hunting can be both proactive and reactive. 
% In the proactive approach, analysts hypothesize potential threats and search for early indicators of attacks without waiting for alerts. 
% In the reactive approach, threat hunting begins in response to specific alerts. Regardless of the trigger, the process involves analyzing IOCs, TTPs, and patterns derived from CTI.
% Tools such as eXtended Detection and Response (XDR) solutions and Security Orchestration, Automation, and Response (SOAR) systems play a critical role in automating parts of the data collection process. 
% Frameworks like MITRE ATT\&CK and the Pyramid of Pain guide analysts in mapping adversary behavior and prioritizing findings. 

% \mypar{Incidence Response.}
% Incident response (IR) and management refer to the organized approach to addressing and managing security incidents to minimize their impact and prevent recurrence. 
% It involves a structured process comprising preparation, detection, containment, eradication, recovery, and post-incident review. 
% The goal is to ensure a timely and effective resolution of incidents while preserving evidence for forensic analysis. 
% CTI like behavior graphs, threat actor attribution, and TTPs help identify the nature and scope of the incident, prioritize response efforts based on threat severity, and guide containment and remediation strategies. 
% By leveraging threat intelligence, organizations can make informed decisions during an incident, improve situational awareness, and enhance the overall effectiveness of their response capabilities. 
% Unlike threat hunting and detection, incident response focuses on managing confirmed incidents rather than searching for or identifying potential threats.

% \mypar{Risk Management.}
% We want to talk about evolving and emerging threats.

% \mypar{Security Awareness and Training.}
% Employee training and awareness, as an application of Cyber Threat Intelligence (CTI), focuses on equipping staff with the knowledge and skills to identify and respond to cyber threats effectively. This involves leveraging CTI to design training programs that reflect real-world threat patterns, incorporating insights into tactics, techniques, and procedures (TTPs) observed in current attacks. Such training may include phishing simulations, scenario-based exercises, and contextual awareness sessions tailored to specific roles within the organization. Industry standards like the NIST Cybersecurity Framework and the NICE Workforce Framework for Cybersecurity emphasize the importance of integrating threat intelligence into workforce development to cultivate a proactive cybersecurity culture. However, despite the growing sophistication of CTI tools, there is a notable lack of automated systems capable of dynamically generating employee awareness alerts or programs based on evolving threat patterns, leaving organizations to manually translate intelligence into training initiatives.

\subsection{Challenges and Opportunities for AI}
\label{ssec:challenges_cti_application}
% In this subsection, we examine the ways AI-based solutions can alleviate practical challenges associated with validating, prioritizing, and applying CTI feeds. 

\mypar{Leveraging Unique and Low-Reputation Feeds.}  
One of the most challenging aspects of CTI triaging is validating intelligence from unique or low-reputation feeds, with over 70\% of practitioners in our survey highlighting validating low-reputed feeds as a significant challenge.
These sources either contain intelligence that is not found in other CTI datasets or originate from providers with little or no historical credibility.  
While such feeds can provide invaluable insights into emerging threats and novel attack vectors, they also pose significant risks.  
Since they lack similarity with other sources, redundancy-based validation is ineffective.  
Similarly, reputation-based validation struggles with low-reputation feeds, as these sources lack a history of verified intelligence.  
Beyond false positives, a more serious concern is adversarial CTI, where malicious actors inject misleading intelligence to poison databases, deceive attribution efforts, or divert forensic investigations~\cite{skopik2020under, ranade2021generating}.  
Due to these risks, analysts are often left with manually analyzing these feeds, a process that is both time-consuming and expertise-dependent.  
% AI presents an opportunity to address these challenges by providing analysts with insights rather than fully automating decisions.  
Our survey results indicate that practitioners prefer LLM-driven assistants for CTI validation (60\%) over fully autonomous validation systems (39\%).  
This suggests a promising direction for semi-autonomous AI agents that support analysts in assessing CTI credibility.  
Recent research has demonstrated the effectiveness of function-calling LLMs in cybersecurity applications, such as penetration testing~\cite{deng2024pentestgpt}.  
Extending this concept to CTI validation, future research could explore agentic frameworks where LLM-driven systems are granted access to multiple intelligence sources, including CVE and CWE databases, structured attack knowledge from MITRE ATT\&CK, and real-time threat intelligence platforms.  
Such an approach would enable LLMs to cross-reference intelligence dynamically, providing analysts with contextual validation insights while mitigating the risk of adversarial CTI.  

\mypar{Determining CTI Relevance and Impact.}  Not all threats pose the same level of risk, making relevance and impact assessment a crucial yet under-explored aspect of CTI triaging.  
Despite its significance, academic research in this area remains limited, leaving organizations to rely on manual evaluations based on attack surface exposure, organizational threat models, and historical telemetry data.  
In our survey, nearly 50\% of practitioners identified prioritizing CTI feeds based on their impact relative to their organization's infrastructure as a key challenge, with a majority highlighting AI as a promising solution for automating this process.  
We believe a promising research direction lies in using LLMs to enhance relevance and impact-based CTI triaging.
By dynamically retrieving organizational data and correlating it with threat intelligence, LLMs can assess a threat’s applicability and potential impact.
Future work could explore assisting analysts in prioritizing intelligence, and ensuring decisions align with an organization’s security posture and risk landscape.  


\mypar{CTI Applicability and Threat Hunting.}  
Existing academic research has primarily focused on leveraging threat intelligence for detection, mapping indicators of compromise to knowledge graphs, and integrating CTI into threat intelligence platforms to assist analysts.  
However, determining whether CTI can be effectively applied within an organization remains an under-explored challenge.  
Organizations operate under resource constraints, and implementing new logging mechanisms to capture relevant threat activity requires significant effort.  
Even when logging systems are in place, analysts often need to manually define and implement detection rules, making CTI operational is a rigorous and time-consuming process.  
In our survey, the majority of practitioners reported using CTI for threat hunting and identified AI as a promising tool for correlating behaviors with TTPs, associating threat intelligence with known threat actors, and countering evasion techniques such as packing.   
Future research could explore leveraging large language models to assess CTI applicability by analyzing an organization's infrastructure, identifying missing logging mechanisms, and even automating detection rule generation.  
Such contributions could streamline threat-hunting capabilities while addressing existing challenges in CTI implementation and reducing manual efforts. 

% \subsection{Applying CTI}
% % Applying Cyber Threat Intelligence (CTI) effectively means transforming validated insights from various threat intelligence feeds into actionable strategies that strengthen an organization's overall cyber defense posture. 
% % Once CTI has been verified and deemed relevant, it becomes a valuable tool to power a range of security initiatives tailored for immediate and long-term needs. 
% % From proactively identifying hidden threats and continuously monitoring systems to building robust long-term defenses and educating employees, CTI empowers organizations to stay ahead of adversaries. 
% % Each of these applications serves a distinct purpose, creating a multi-layered defense strategy that combines immediate response capabilities with forward-looking prevention measures.

% After prioritization and validation, Cyber Threat Intelligence (CTI) from various feeds and sources is transformed into actionable strategies that enhance an organization's cyber defense posture. 
% These strategies leverage CTI to address specific cybersecurity needs and often involve integrating Security Information and Event Management (SIEM) systems to centralize and analyze logs.
% These strategies include using CTI to improve threat detection, which focuses on identifying and mitigating potential threats before they can cause harm, thereby strengthening the organization’s defenses. 
% CTI also plays a pivotal role in incident response management, where contextual intelligence is provided to efficiently handle and remediate security breaches, reducing their impact and ensuring faster recovery. 
% Additionally, CTI supports threat hunting, a proactive approach that uncovers hidden adversaries within the organization’s network, offering enhanced visibility and preemptive control over potential vulnerabilities.
% Moreover, CTI is essential in fraud prevention, which helps organizations detect and prevent fraudulent activities that could compromise their financial or reputational assets. 
% Finally, CTI fosters security awareness and training by educating employees on emerging threats and equipping them with the knowledge to follow best practices, cultivating a strong and secure organizational culture. 
% In the following, we explain each of these strategies in detail.

% \mypar{Threat Detection.}
% Organizations scan for IOCs including IP address, domain names, file hashes, registry key paths associated with threats within their networks and systems, enabling early detection of potential breaches before they escalate. 
% This proactive approach reduces risks and minimizes the likelihood of significant damage. 
% Security Information and Event Management (SIEM) systems are used to monitor and analyze threats in real-time.
% Threat detection often relies on platforms such as Threat Intelligence Platforms (TIPs), which ingest, analyze, and correlate threat intelligence with operational data.
% TIPs use IOCs—such as malicious IP addresses, domain names, or file hashes—to identify potential threats in real time by matching these indicators against system logs, audit trails, or live traffic.
% For instance, platforms like those proposed by Milajerdi et al.\cite{milajerdi2019poirot} and Gao et al.\cite{gao2021system} leverage threat intelligence and kernel-level audit data to align attack behaviors and efficiently detect threats through behavioral analysis and correlation.
% These approaches enable organizations to process large-scale data and uncover sophisticated attack techniques. 
% Similarly, modern frameworks employing machine learning, such as the one by Khan et al.~\cite{khan2021new}, enhance threat detection by leveraging deep learning to discover threats in Industrial IoT (IIoT) networks.

% \mypar{Threat Hunting.} 
% Unlike \textbf{threat detection}, which focuses on using individual Indicators of Compromise (IOCs) and Tactics, Techniques, and Procedures (TTPs) to make real-time decisions, threat hunting leverages this intelligence as a starting point to identify unknown threats.
% Cybersecurity experts often debate the exact stages of the threat hunting cycle and its classification as reactive versus proactive \cite{maxam2024interview}. 
% Some define it as proactively searching for early indications of ongoing attacks without waiting for alerts \cite{rastogi2023cyber}. 
% Others describe it as an investigative process triggered by alerts. 
% The distinction lies in the investigation's trigger, yet both forms aim to uncover undetected threats within an organization’s network, guided by intelligence.
% Threat hunting is exploratory, human-driven, and hypothesis-based, enabling analysts to uncover sophisticated threats that evade automated detection systems. 
% Analysts employ tools such as eXtended Detection and Response (XDR) solutions and Security Orchestration, Automation, and Response (SOAR) systems to partially automate data collection. 
% Numerous frameworks have been proposed, including the MITRE ATT\&CK framework \cite{mitre_attack}, the Pyramid of Pain \cite{bianco2013pyramid}, and others, to categorize adversary activity and focus threat hunting efforts. 
% Recent advancements in Natural Language Processing (NLP) have enhanced threat hunting by extracting attack information from online forums \cite{zhu2018chainsmith}, open-source cyber threat intelligence (OSCTI) feeds \cite{gao2021enabling}, and threat reports \cite{dekel2022mabat, alam2023looking, Rani2024TTPXHunterAT, kaiser2023attack}. 
% These techniques convert data into machine-readable formats \cite{Rani2024TTPXHunterAT}, build knowledge bases, identify attack patterns \cite{gao2021enabling, alam2023looking, kaiser2023attack}, and prioritize artifacts for analysis \cite{dekel2022mabat}.
% Even though AI-driven systems have advanced in mapping low-level indicators to high-level behavioral patterns like TTPs, their integration into analyst workflows with a focus on interpretability and explainability remains a challenge. 
% Addressing this could further enhance the effectiveness and trustworthiness of threat hunting methodologies.


% \mypar{Incidence Response Management.}
% Incident response and recovery focus on detecting, analyzing, containing, and remediating active threats to minimize damage. Threat intelligence provides critical information about the nature, scope, and severity of incidents. It helps organizations isolate affected systems, identify the attacker’s methods, and implement steps to recover from the attack.

% Information extracted from CTI improves an analyst’s ability to recognize relevant threats and
% respond to them in a timely manner. This is, methods for CTI analysis can provide analysts with a list of related information, supporting their decision-making as they handle cyber incidents

% \mypar{Fraud Prevention.}

% \mypar{Security Awareness and Training.}
% Employee training and awareness, as an application of Cyber Threat Intelligence (CTI), focuses on equipping staff with the knowledge and skills to identify and respond to cyber threats effectively. This involves leveraging CTI to design training programs that reflect real-world threat patterns, incorporating insights into tactics, techniques, and procedures (TTPs) observed in current attacks. Such training may include phishing simulations, scenario-based exercises, and contextual awareness sessions tailored to specific roles within the organization. Industry standards like the NIST Cybersecurity Framework and the NICE Workforce Framework for Cybersecurity emphasize the importance of integrating threat intelligence into workforce development to cultivate a proactive cybersecurity culture. However, despite the growing sophistication of CTI tools, there is a notable lack of automated systems capable of dynamically generating employee awareness alerts or programs based on evolving threat patterns, leaving organizations to manually translate intelligence into training initiatives.

% \subsection{Threat Intelligence Platforms}

% The process of ingesting, triaging, and applying CTI is challenging due to the volume of the data and the dynamic nature of both the threat landscape and the network infrastructure of an organization.

% To help in these tasks, Threat Intelligence Platforms (TIPs) provide support to the SOC analyst in carrying out CTI-related tasks. 
% While there are a number of commercial offerings, the MISP project~\cite{Wagner2016MISPTD} has established itself as the de facto standard for open-source intelligence platforms. 

% First and foremost, TIPs provide centralized storage for multiple streams of CTI data (such as IoC feeds, blog posts, reports, and alerts).
% These feeds are often consumed through feed-specific plugins whose task is to extract relevant information, which is then encoded in a common schema or ontology.
% This task is relatively simple when CTI is in machine-readable format, but it can become challenging when threat-related information is described in natural language or as unstructured log data.
% In these cases, LLM-based techniques could be used to parse the data using pre-existing knowledge about the ontology being used to represent the data, using approaches similar to the ones used to generate CTI from unstructured data~\cite{gao2021system}.
% Once the data is ingested, TIPs provide means of correlating the data, for example by connecting two reports that mention the same malware sample hash or that refer to the same domain name.

% A second common use of TIPs is through integration with software inventory and vulnerability scanning tools.
% These tools provide a view of the components and services deployed in an infrastructure, which allows a TIP to identify CTI data that is highly relevant to a specific infrastructure, allowing for effective CTI triaging.
% The simplest approach matches the vulnerable products mentioned in a CVE record mentioned in a report with the software deployed in the organization's network, but AI could enable more sophisticated processing where the multi-step attack patterns mentioned in a threat report are directly mapped to an infrastructure's components to understand the feasibility of a similar attack in the local context.

% Another common application of TIPs is through integration with malware analysis environment and signature evaluation system. 
% In this case the goal is to answer the question: ``If this attack would happen in my infrastructure, would I be able to detect it?''
% Automating this task is challenging, as it requires the automatic downloading of malicious artifacts, the reproduction of network-based attacks, and the analysis of the combined results. 
% Approaches based on LLM agents have shown promise in the creation of exploits, but more work needs to be done to effectively leverage CTI data to automatically determine the detection efficacy and threat coverage of an organization's security infrastructure.

% The fourth application of TIPs is the use of CTI for threat hunting in the local context.
% By integrating with the logs collected by network and host monitoring tools (often stored in large log management systems) with CTI, it is possible to support the identification of attacks in an organization's network based on information contained in CTI reports.
% This is the main goal of CTI itself: using pre-existing information about cyber threats to detect and mitigate the attacks in an organization's network.
% At the moment this is largely a manual process, and TIPs work as support for SOC analysts and threat hunters.
% However, there is a great opportunity to use AI-based techniques in order to enhanced manual analysis (e.g., by providing a RAG-based contextualization of network events based on CTI) or to automatically understand if the evidence of instances of attacks described in CTI feeds is actually present in an organization's network. 


% Challenges: (1) Effective threat hunting requires robust monitoring capabilities and specialized tools, which can be resource-intensive to develop and maintain. 
% (2) Different TI feeds may provide IOCs in different formats. Therefore one needs to generalize these feeds before applying them.


%  \textbf{Threat Attribution}
% Attribution refers to identifying the individuals or groups responsible for malicious activities. 
% Utilizing CTI, organizations analyze tactics, techniques, and procedures (TTPs) associated with an attack to link it to known threat actors. 
% This involves examining malware characteristics, attack vectors, and other IOCs to build a profile of the attacker.
% Example: Attributing a program behavior to Mitre Tactics and Techniques, using code similarity to attribute code to a certain nation-state threat actor.

% Challenges: 
% (1): Attribution is complex due to sophisticated obfuscation methods used by threat actors.
% (2): Multi-process attribution is still a challenge

% Potential Use of AI: 
% Perform multi-process threat attribution

% \textbf{Security Awareness and Internal training}
% CTI can be used to develop security awareness and training programs for employees, helping them recognize and respond to potential security incidents. 

% \subsubsection{Opportunities for AI}
% \sv{Normalizing feeds from different TI sources?}

% \textbf{Threat Correlation}
% Threat correlation involves identifying relationships between various data points or events to uncover potential threats. 
% In context to CTI, this means analyzing different sources of information to detect patterns or trends that might indicate malicious activity. 
% For example, correlating multiple failed login attempts from unusual geographic locations with increased outbound traffic to known malicious domains can reveal a coordinated attack.

% Challenges: Same as Threat hunting
% Potential use of AI: Same as threat hunting


%  \textbf{Threat Attribution}
% Attribution refers to identifying the individuals or groups responsible for malicious activities. 
% Utilizing CTI, organizations analyze tactics, techniques, and procedures (TTPs) associated with an attack to link it to known threat actors. 
% This involves examining malware characteristics, attack vectors, and other IOCs to build a profile of the attacker.
% Example: Attributing a program behavior to Mitre Tactics and Techniques, using code similarity to attribute code to a certain nation-state threat actor.

% Challenges: 
% (1): Attribution is complex due to sophisticated obfuscation methods used by threat actors.
% (2): Multi-process attribution is still a challenge

% Potential Use of AI: 
% Perform multi-process threat attribution

% \textbf{Threat Prioritization}:
% Organizations prioritize threats based on their potential impact, ensuring resources address the most significant risks. 
% This involves assessing the likelihood and potential damage of different threat scenarios, considering factors like data sensitivity and system criticality.

% \jc{\textbf{Integration to IDS:} Integrate validated CTI to the deployed IDS's database (e.g., newly detected malware signatures, botnet IPs) to mitigate potential similar attacks in the future.
% }

==> Sections/07_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Other works that attempted to systematize CTI should go here.
What did they try to accomplish? How are they different from the framework we propose? Why are we better?

A more nuanced assesment of CTI quality has been proposed by related work~\cite{sakellariou_methodology_2024}, however the evaluation of it's application is beyond the scope of this paper.

==> Sections/clipboard.tex <==
Codification serves three primary purposes: (1) converting the intelligence into a format aligned with the sharing medium, (2) incorporating safeguards to ensure the data shared is compliant with regulations and policies, and (3) establishing a common understanding and reference between CTI providers and recipients. 

The first step in codification transforms the raw intelligence into a structured or unstructured format. 
Structured formats are designed for automated systems, enabling seamless integration into security tools and workflows. 
Unstructured formats, such as natural language summaries, target human audiences and are often shared through blogs, reports, or forums. 
The choice of format depends on the sharing medium.

When CTI is shared outside an organization, safeguards must be applied so that the shared intelligence does not inadvertently expose sensitive organizational details or violate privacy regulations. 
Safeguarding filters out identifiable information, sanitizes organizational specifics, and ensures that published CTI adheres to established guidelines for secure sharing. 
Although the shared intelligence itself may require further validation and refinement by recipients, the process of codification ensures that it is comprehensible, well-organized, and primed for collaborative use.


% \subsection{Sharing/Distribution of CTI (Hadjer)}
% % Ways to share 
% % diffrent meduims for sharing
% % challenges
% % ML opportunities
% This paper \cite{geras2023sharing} discusses TI sharing platforms from a user's perspective. 
% GV:I also found this~\cite{zibak19:sharing} but have not read it...
% Interesting as well: "Threat intelligence sharing platforms: An exploratory study of software vendors and research perspectives."

% \takeaway{Sharing CTI is critical to the collective effort of cybersecurity, enabling an exchange of knowledge within trusted organizations, distribution within the security community, or publication to a broader audience.
% This forms a collective library of knowledge that security experts can utilize in their fight against attackers.
% By distributing CTI, organizations can coordinate responses to develop robust defenses against emerging threats.}


==> Sections/llm_usage_considerations.tex <==
\section*{LLM usage considerations}

All text and figures in this paper were created exclusively by the authors.
Where LLMs were used during writing, their role was limited to grammar-suggestion and style-suggestion tools, and all suggestions were manually reviewed and accepted by an author. LLMs were also used to assist in implementing parts of the experimental workflow; however, any generated code underwent the same validation and testing procedures as code written by a human developer.

% \mypar{Transparency.}
% LLMs are central to the experiments in this SoK. 
% Because individual LLM queries can be non-deterministic, we designed a structured output format for each experiment, and the LLM responses required the model to provide, for every CTI insight, its supporting evidence and reasoning. 
% % Furthermore, we incorporated LLM-State management (short-term memory) which further keeps the analysis directed 
% We found that enforcing this structure greatly improved the consistency and interpretability of model responses.
% We note that proprietary LLMs evolve, which may affect exact reproducibility. 
% However, as underlying models advance, both exact results and error profiles may change; future work should re-evaluate these trends over time.

% \mypar{Responsibility.}
% % Model selection was performed using a dedicated validation set (see~\autoref{sec:experimental-setup}). 
% Several LLMs were evaluated, and the model offering the best cost–performance tradeoff was chosen for all subsequent experiments.

==> Sections/motivating_example.tex <==
% \section{Motivating Example}


% This motivating example illustrates the critical role of the CTI lifecycle—from generating actionable insights, to sharing them in an accessible and secure manner, and finally applying them to enhance security postures. 
% By leveraging collaboration and prioritizing intelligence effectively, organizations can build a robust defense against evolving cyber threats. 
% This cyclical process not only protects individual organizations but also fosters a collective effort to safeguard the broader cybersecurity landscape.

==> Tables/datasets.tex <==
\begin{table}[t!]
\centering
\small
\caption{Summary of Curated Datasets for Experiments.}
\label{table:dataset-summary}
\begin{tabular}{l l l}
\toprule
\textbf{Dataset Source} & \textbf{Dataset Name} & \textbf{Format} \\
\midrule
DARPA E3 & Cadet, Trace, Five Directions & CSV \\
DARPA E5 & Cadet, Trace, Five Directions & CSV \\
Proprietary & Black-suit Ransomware & JSON \\
& Nitrogen Campaign & JSON \\
& Egg-celent Resume & JSON \\
Malware Sandbox & 55 Malware Samples & JSON, XML \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/logs_to_activity.tex <==
\usepackage{booktabs} % For professional lines
\usepackage{tabularx} % For auto-fitting to column width

\begin{table}[h]
\centering
\caption{Extracting malicious indicators: Malicious Behaviors, and IoCs}
\label{table:performance}
\small % Slightly smaller font often helps in narrow columns
\begin{tabularx}{\columnwidth}{@{} l *{3}{C} @{}}
\toprule
\textbf{Campaign ID} & \textbf{GT} & \textbf{GPT-4} & \textbf{Claude} & \textbf{D-Seek} \\
\midrule
23634 (BlackSuit)   & 12 & 11 & 11 & 11 \\
27244 (LockBit)     & 14 & 13 & 10 & 11 \\
27899 (FIN6)        & 13 & 11 & 11 & 8  \\
25590 (BlackCat)    & 14 & 12 & 13 & 12 \\
\midrule
\textbf{Total (53)} & \textbf{100\%} & \textbf{88.6\%} & \textbf{84.9\%} & \textbf{79.2\%} \\
\bottomrule
\end{tabularx}
\end{table}

==> Tables/validation_result.tex <==
\begin{table}[ht]
\centering
\caption{Validation Results for Model Selection.}
\label{table:validation-results}
\begin{tabular}{l c c c c}
\toprule
\textbf{Model} & \textbf{Exp. 1} & \textbf{Exp. 2} & \textbf{Exp. 3} & \textbf{Exp. 4} \\
\midrule
GPT-5-mini Medium & X & X & X & X \\
Claude Haiku 4.5 & X & X & X & X \\
Qwen 235B Instruct & X & X & X & X \\
\bottomrule
\end{tabular}
\end{table}
